The Fault in our Stars: Quality Assessment of Code Generation Benchmarks

Large Language Models (LLMs) are gaining popularity among software engineers. A crucial aspect of developing effective code generation LLMs is to evaluate these models using a robust benchmark. Evaluation benchmarks with quality issues can provide a false sense of performance. In this work, we conduct the first-of-its-kind study of the quality of prompts within benchmarks used to compare the performance of different code generation models. To conduct this study, we analyzed 3,566 prompts from 9 code generation benchmarks to identify quality issues in them. We also investigated whether fixing the identified quality issues in the benchmarks' prompts affects a model's performance. We also studied memorization issues of the evaluation dataset, which can put into question a benchmark's trustworthiness. We found that code generation evaluation benchmarks mainly focused on Python and coding exercises and had very limited contextual dependencies to challenge the model. These datasets and the developers' prompts suffer from quality issues like spelling and grammatical errors, unclear sentences to express developers' intent, and not using proper documentation style. Fixing all these issues in the benchmarks can lead to a better performance for Python code generation, but not a significant improvement was observed for Java code generation. We also found evidence that GPT-3.5-Turbo and CodeGen-2.5 models may have data contamination issues.

==> Codes/P12_interogation.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{\textbf{Dataset}: NumpyEval\cite{zan2022cert}. \textbf{Prompt ID}: 95}}}
import numpy as np

a = np.array([1,2,3,4,5,6])
b = np.array([1,4,5])

# Is there a way to compare what elements in a exist in b?
# Return a array of booleans, True if elements in a exist in b, False otherwise
c =
\end{PythonSourceCode*}
}
% \vspace{-10pt}
\caption{Example of interrogation in prompt}\label{lst:P12_interogation}
\end{listing}
% https://jdasilv2.pythonanywhere.com/datasets_study/prompts/2255

==> Codes/P13_bad_JavaDoc.tex <==

\begin{listing}[H]
{
\begin{JavaSourceCode*}{label=\textcolor{black}{\tiny{\textbf{Dataset}: MBXP\textsubscript{MathQA}~\cite{athiwaratkun2023multilingual}. \textbf{Prompt ID}: 249}}}

import java.io.*;
import java.lang.*;
import java.util.*;
import java.math.*;


class Problem \{

    /**
     * machine a produces 100 parts thrice as fast as machine b does . machine b produces
     100 parts in 30 minutes . if each machine produces parts at a constant rate , how many
     parts does machine a produce in 6 minutes ? n0 = 100.0 n1 = 100.0 n2 = 30.0 n3 = 6.0
     */
    public static double problem() \{

\end{JavaSourceCode*}
}
\caption{Example of bad JavaDoc}\label{lst:P13_bad_JavaDoc}
\end{listing}

%https://jdasilv2.pythonanywhere.com/datasets_study/prompts/1744



==> Codes/P13_standard_JavaDoc.tex <==

\begin{listing}[H]
{
\begin{JavaSourceCode*}{label=\textcolor{black}{\tiny{\textbf{Dataset}: MBXP\textsubscript{HumanEval}~\cite{athiwaratkun2023multilingual}. \textbf{Prompt ID}: 159}}}


    /**
     * * You're a hungry rabbit, and you already have eaten a certain number of carrots,
     * but now you need to eat more carrots to complete the day's meals.
     * you should return an array of [ total number of eaten carrots after your meals,
     *                                 the number of carrots left after your meals ]
     * if there are not enough remaining carrots, you will eat all remaining carrots, 
     * but will still be hungry.
     * 
     * Example:
     * * eat(5, 6, 10) -> [11, 4]
     * * eat(4, 8, 9) -> [12, 1]
     * * eat(1, 10, 10) -> [11, 0]
     * * eat(2, 11, 5) -> [7, 0]
     * 
     * Variables:
     * @param number: 
     * @param need
     * @param remaining
     * @return;...
     * 
     * Constrain:
     * * 0 <= number <= 1000
     * * 0 <= need <= 1000
     * * 0 <= remaining <= 1000

     * Have fun :)
     *
     */

\end{JavaSourceCode*}
}
\caption{Example of a standard JavaDoc}\label{lst:P13_standard_JavaDoc}
\end{listing}

%https://jdasilv2.pythonanywhere.com/datasets_study/prompts/1744



==> Codes/P15_unclear.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\sf\tiny{\textbf{Dataset}: TorchDataEval~\cite{zan2022language}. \textbf{Prompt ID}: 17}}}
import monkey as mk
import numpy as np
kf = mk.KnowledgeFrame({'a': [4, 1, 7, 3], 'b': [5, 2, 9, 6], 'c': [6, 3, 2, 8]})
# I would like to create new knowledgeframe out of the old one in a way that 
# there will only be values that exceed the average value of the column. 
# We can compare values and then add NaNs by indexing or `where`
# We want remove NaNs also in first rows add custom function with `sipna`
kf = 
\end{PythonSourceCode*}
}
% \vspace{-10pt}
\caption{Example of a unclear intention.}\label{lst:P15_example_unclear}
\end{listing}


==> Codes/P6_example_gib.tex <==
\begin{listing}[H]
\renewcommand\theFancyVerbLine{%
    \ifnum\value{FancyVerbLine}=4
        \sf\setcounter{FancyVerbLine}{11}\color[rgb]{0,0,0}\ldots
    \else
    \sf\textcolor[rgb]{0,0,0}{\tiny\arabic{FancyVerbLine}}%
    \fi
}
\begin{PythonSourceCode*}{label=\textcolor{black}{\sf\tiny{\textbf{Dataset}: HumanEval~\cite{chen2021evaluating}. \textbf{Prompt ID}: 94}}}
def skjkasdkd(lst):
    """You are given a list of integers.
    You need to find the largest prime value and return the sum of its digits.

    """
\end{PythonSourceCode*}
% \vspace{-10pt}
\caption{Example of gibberish function name}\label{lst:P6_example_gib}
\end{listing}
% 84


==> Codes/P6_example_wrong.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{below\_zero.py}}}

def solve(N):
    """Given a positive integer N, return the total sum of its digits in binary.
    
    Example
        For N = 1000, the sum of digits will be 1 the output should be "1".
        For N = 150, the sum of digits will be 6 the output should be "110".
        For N = 147, the sum of digits will be 12 the output should be "1100".
    
    Variables:
        @N integer
             Constraints: 0 \leq N \leq 10000.
    Output:
         a string of binary number
    """


\end{PythonSourceCode*}
}
\caption{Example of wrong function name}\label{lst:P6_example_wrong}
\end{listing}
% 94

==> Codes/P8_different_inout.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{below\_zero.py}}}

def make_a_pile(n):
    """
    Given a positive integer n, you have to make a pile of n levels of stones.
    The first level has n stones.
    The number of stones in the next level is:
        - the next odd number if n is odd.
        - the next even number if n is even.
    Return the number of stones in each level in a list, where element at index
    i represents the number of stones in the level (i+1).

    Examples:
    >>> make_a_pile(3)
    [3, 5, 7]
    """


\end{PythonSourceCode*}
}
\caption{Example of different number of input-output pair}\label{lst:P8_different_inout}
\end{listing}

% 100

==> Codes/P8_different_style.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{below\_zero.py}}}




\end{PythonSourceCode*}
}
\caption{Example of different number of input-output pair}\label{lst:P8_different_style}
\end{listing}

% 100

==> Codes/P8_typeHint.tex <==



\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{below\_zero.py}}}

def remove_vowels(text):
    """
    remove_vowels is a function that takes string and returns string without vowels.
    >>> remove_vowels('')
    ''
    >>> remove_vowels("abcdef\nghijklm")
    'bcdf\nghjklm'
    >>> remove_vowels('abcdef')
    'bcdf'
    >>> remove_vowels('aaaaa')
    ''
    >>> remove_vowels('aaBAA')
    'B'
    >>> remove_vowels('zbcd')
    'zbcd'
    """


\end{PythonSourceCode*}
}
\caption{Example of not giving type hint in python}\label{lst:P8_typeHint}
\end{listing}
% 51



==> Codes/P9_url_example.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\sf\tiny{\textbf{Dataset}: MBPP~\cite{MBPP}. \textbf{Prompt ID}: 420}}}
def is_perfect_square(n):
   """
   Write a function to check whether the given number is a perfect square or not. 
   https://www.geeksforgeeks.org/check-if-given-number-is-perfect-square-in-cpp/
   """
\end{PythonSourceCode*}
}
% \vspace{-10pt}
\caption{Example of having URL in the prompt.}\label{lst:P9_example_url}
\end{listing}


==> Codes/inconsitant.tex <==


\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\sf\tiny{\textbf{Dataset}: HumanEval~\cite{HumanEval}. \textbf{Prompt ID}: 132}}}
def is_nested(string):
    '''
    Create a function that takes a string as input which contains only square brackets.
    The function should return True if and only if there is a valid subsequence of brackets 
    where at least one bracket in the subsequence is nested.

    is_nested('[[]]') -> True
    is_nested('[]]]]]]][[[[[]') -> False
    is_nested('[][]') -> False
    is_nested('[]') -> False
    is_nested('[[][]]') -> True
    is_nested('[[]][[') -> True
    '''
\end{PythonSourceCode*}
}
\caption{Example of a unclear intention.}\label{lst:inconsistant}
\end{listing}



==> Codes/p1_example.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{below\_zero.py}}}
from typing import List

def below_zero(operations: List[int]) -> bool:
    """ 
    You're given a list of deposit and withdrawal operations 
    on a bank account that starts with zero balance. 
    Your task is to detect if, at any point, 
    the balance of the account fallls below zero, and
    at that point, the function should return True. 
    Otherwise, it should return False.
    >>> below_zero([1, 2, 3])
    False
    >>> below_zero([1, 2, -4, 5])
    True
    """
\end{PythonSourceCode*}
}
\caption{Example of Spelling Error}\label{lst:p1_example}
\end{listing}

==> Codes/p1_example_false_pos.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{below\_zero.py}}}
def change_base(x: int, base: int):
    """Change numerical base of input number x to base.
    return string representation after the conversion.
    base numbers are less than 10.
    >>> change_base(8, 3)
    '22'
    >>> change_base(8, 2)
    '1000'
    >>> change_base(7, 2)
    '111'
    """
\end{PythonSourceCode*}
}
% \vspace{-10pt}
\caption{Example of a False Positive Spelling Error}\label{lst:p1_example_false_pos}
\end{listing}

==> Codes/p3_example.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\sf\tiny{\textbf{Dataset:} MathQA~\cite{MBXP}. \textbf{Prompt ID:} 94.}}}
def problem():
    """
    a train is 410 meter long is running at a speed of 45 km / hour . in what time will it 
    pass a bridge of 140 meter length n0 = 410.0 n1 = 45.0 n2 = 140.0
    """
\end{PythonSourceCode*}
}
% \vspace{-10pt}
\caption{Example of a prompt with an incomplete sentence}\label{lst:p3_example}
\end{listing}

==> Codes/p4_example.tex <==
\begin{listing}[H]
{
\begin{PythonSourceCode*}{label=\textcolor{black}{\tiny{below\_zero.py} \hl{replace with Dataset name and prompt ID in here}} }
FIX = """
Add more test cases.
"""

def vowels_count(s):
    """Write a function vowels_count which takes a string representing a word as input and 
    returns the number of vowels in the string. Vowels in this case are 'a', 'e', 'i', 'o', 
    'u'. Here, 'y' is also a vowel, but only when it is at the end of the given word.

    Example:
    >>> vowels_count("abcde")
    2
    >>> vowels_count("ACEDY")
    3
    """
\end{PythonSourceCode*}
}
\caption{Example of Self Admitted Technical Debt}\label{lst:p4_example}
\end{listing}
